CodeRepoQA: A Large-scale Benchmark for Software Engineering Question Answering

In this work, we introduce CodeRepoQA, a large-scale benchmark specifically designed for evaluating repository-level question-answering capabilities in the field of software engineering. CodeRepoQA encompasses five programming languages and covers a wide range of scenarios, enabling comprehensive evaluation of language models. To construct this dataset, we crawl data from 30 well-known repositories in GitHub, the largest platform for hosting and collaborating on code, and carefully filter raw data. In total, CodeRepoQA is a multi-turn question-answering benchmark with 585,687 entries, covering a diverse array of software engineering scenarios, with an average of 6.62 dialogue turns per entry. We evaluate ten popular large language models on our dataset and provide in-depth analysis. We find that LLMs still have limitations in question-answering capabilities in the field of software engineering, and medium-length contexts are more conducive to LLMs' performance. The entire benchmark is publicly available at https://github.com/kinesiatricssxilm14/CodeRepoQA.

==> tables/base_info.tex <==
\begin{table}[t]
    \centering
    \caption{Basic information for each entry in GitHub issues and pull requests, including Base Information, Content Information, and Pull Request-Specific Details.}
        \centering
        % \small
        \footnotesize
        % \fontsize{10}{11}\selectfont
        % \normalsize
        \setlength{\tabcolsep}{1.5mm} % 进一步减少表格单元之间的距离
        \renewcommand{\arraystretch}{1.0}
        \begin{tabular}{c p{9.2cm}} % 调整第二列宽度以适应整体宽度
            \toprule
             \textbf{Features} &  \textbf{Description} \\ \midrule
            \multicolumn{2}{c}{\textbf{Base Information}} \\ \midrule
            language &  The primary programming language used in the repository.\\
            type &  Whether the entry is an Issue or a PR. \\
            repo &  The repository's name. \\
            owner &  The repository owner, either an individual or an organization. \\
            number &  The unique identifier for the issue or PR. \\
            author-info &  Details about the author of the issue or PR. \\
            author-association &  The author's relationship with the repository (e.g., member).\\
            state &  The current status of the issue or PR (e.g., open, closed). \\
            created-at &  The timestamp when the issue or PR was created. \\
            updated-at &  The timestamp of the most recent update to the issue or PR. \\
            \midrule
            \multicolumn{2}{c}{\textbf{Content Information}} \\ \midrule
            title &  The title of the issue or PR. \\
            body &  The main content or description of the issue or PR. \\
            comments &  The content of comments on the issue or PR. \\
            \midrule
            % \multicolumn{2}{c}{\textbf{Interaction Information}} \\ \midrule
            % labels &  Tags or labels assigned to the issue or PR to categorize them. \\
            % milestones &  Grouping of issues or PRs based on timelines or project phases. \\
            % assignees &  Individuals assigned to handle the issue or PR. \\
            % reactions &  Reactions to the issue or PR, such as +1, -1, heart, etc. \\
            % events &  Actions and state changes tracking of the issue or PR. \\
            % \midrule
            \multicolumn{2}{c}{\textbf{Pull Request-Specific Details}} \\ \midrule
            merged &  Whether the PR has been merged. \\
            base-info & Information about the base branch of the PR. \\
            head-info & Information about the head branch of the PR. \\
            patch &  The patch details of the PR, describing the changes made. \\
            review-comments & Comments or feedback provided during the PR review process. \\
            \bottomrule
        \end{tabular}
        \label{tab:dataset_info}
    \end{table}

==> tables/models.tex <==
\definecolor{darkgreen}{rgb}{0,0.5,0}

\begin{table}[t]
    \caption{Selected LLMs, where "-" indicates unknown.}
    \footnotesize
    \renewcommand{\arraystretch}{0.9}
    \centering
    \setlength{\tabcolsep}{1.2mm}
    \begin{tabular}{c|ccc}
    \toprule
    \textbf{Model} & \textbf{Size} & \textbf{Instruct} & \textbf{Open-source}
\\
\midrule
GPT-4o
& -
& \cross
& \cross
\\
GPT-4
& -
& \cross
& \cross
\\
Gemini-1.5-Flash
& -
& \cross
& \cross
\\
Gemini-1.5-Pro
& -
& \cross
& \cross
\\
\midrule
Mistral-large-2
& 123B
& \tick
& \tick
\\
CodeQwen-1.5-Chat
& 7B
& \tick
& \tick
\\
DeepSeek-Coder-V2
& 236B
& \tick
& \tick
\\
DeepSeek-Coder-V2-Lite
& 16B
& \tick
& \tick
\\
DeepSeek-Coder
& 33B
& \tick
& \tick
\\
DeepSeek-Coder
& 6.7B
& \tick
& \tick
\\
    \bottomrule
    \end{tabular}
    \label{tab:models}
\end{table}
